VelServe: Taming Decode Jitters in LLM Inference with Tail-Calibrated Scheduling

Interactive LLM services must meet latency service-level objectives (SLOs) for the time to first token (TTFT) and the time between tokens (TBT), as streaming and soft real-time applications require predictable token delivery. We identify decode jitters in both aggregated and disaggregated serving. A jitter delays every request in the batch, and long responses span hundreds of steps, so even rare overruns cause many SLO violations. In aggregated serving, SLO-aware schedulers set each step's prefill budget until its predicted latency just meets the TBT target, leaving no room for mispredictions or host stalls. Disaggregation meets average TBT targets at a cost in capacity, yet the steps that admit new requests still run late. We present \sysname, a scheduler that calibrates how much prefill work each decode step carries using the measured tail of its own iteration latency. The SLO determines how rare a late step must be, and \sysname leaves enough headroom in each iteration to prevent overruns and meet the target decode latency. This headroom slows prefill, so \sysname serves the shortest waiting prompt first. When TTFT deadlines grow with prompt length, the long prompts it delays have the most time to spare. Under disaggregation, it spaces admissions so that no request waits on more slow admission steps than its P99 target allows. On three attention families and varying workloads, \sysname sustains 2.4--2.9$\times$ the SLO goodput of the strongest baseline on Qwen3-8B and DeepSeek-V4-Flash, and at least 4.4$\times$ on DeepSeek-V2-Lite. With prefill and decode disaggregated on eight GPUs, \sysname meets the SLO for more than twice as many requests as state-of-the-art baselines.

==> figures/ds_overrun.tex <==
Qwen3-8B & Niyama & 1.71 & 2.15 & +1.1 & 16 \\
 & Medha & 0.00 & 1.36 & +4.9 & 20 \\
 & \sysname & 0.00 & 0.00 & +1.0 & 16 \\
\midrule
V2-Lite & Niyama & 1.00 & 1.11 & +2.4 & 125 \\
 & Medha & 0.00 & 1.60 & -1.2 & 25 \\
 & \sysname & 0.00 & 0.01 & -3.2 & 16 \\
\midrule
V4-Flash & Niyama & 8.37 & 12.40 & -4.5 & 5 \\
 & Medha & 0.00 & 3.97 & +0.1 & 9 \\
 & \sysname & 0.00 & 0.02 & +0.2 & 5 \\

